Causal Fairness Analysis

Decision-making systems based on AI and machine learning have been used throughout a wide range of real-world scenarios, including healthcare, law enforcement, education, and finance. It is no longer far-fetched to envision a future where autonomous systems will be driving entire business decisions and, more broadly, supporting large-scale decision-making infrastructure to solve society's most challenging problems. Issues of unfairness and discrimination are pervasive when decisions are being made by humans, and remain (or are potentially amplified) when decisions are made using machines with little transparency, accountability, and fairness. In this paper, we introduce a framework for \textit{causal fairness analysis} with the intent of filling in this gap, i.e., understanding, modeling, and possibly solving issues of fairness in decision-making settings. The main insight of our approach will be to link the quantification of the disparities present on the observed data with the underlying, and often unobserved, collection of causal mechanisms that generate the disparity in the first place, challenge we call the Fundamental Problem of Causal Fairness Analysis (FPCFA). In order to solve the FPCFA, we study the problem of decomposing variations and empirical measures of fairness that attribute such variations to structural mechanisms and different units of the population. Our effort culminates in the Fairness Map, which is the first systematic attempt to organize and explain the relationship between different criteria found in the literature. Finally, we study which causal assumptions are minimally needed for performing causal fairness analysis and propose a Fairness Cookbook, which allows data scientists to assess the existence of disparate impact and disparate treatment.

==> measures.tex <==
\section{TV family} \label{Measures}
In this section, we introduce a family of measures that populate the explainability plane. Since all the measures describe variations included within the TV measure, we refer to them as the \textit{TV family} (part $e$ of Fig.~\ref{fig:roadmap}). These measures are essential for performing Causal Fairness Analysis, and as we show in the Fairness Map (Thm.~\ref{thm:map}), they form hierarchy in terms of power, admissibility and decomposability relations.  

\subsection{From population to unit} \label{MeasuresGap}
After introducing our theoretical framework and the two axes explainability plane, we are ready to instantiate a number of causal fairness measures. The measures are introduced in order, starting from measures that quantify discrimination in the entire population of units $u$ (corresponding to posterior $P(u)$), and reaching measures that quantify discrimination for a single unit $u$ (corresponding to the posterior $\delta_u$, where $\delta$ is the Dirac delta function).

\subsubsection{Population level - \(P(u)\)}
As was noted earlier, TV captures the difference between groups generated by any mechanism of association (both causal and non-causal). Therefore, in the first step, we distinguish between causal and non-causal (or spurious) mechanism. 
% \begin{wrapfigure}{r}{0.50\textwidth}
% \centering
% 	\begin{tikzpicture}[gap]
	
% 	    % nodes
%         \node [f1] (data) at (5, 12) {Data $\mathcal{D}$};
% 		\node [f2] (tv) at (5, 11) {TV};
		
% 		\node [f2] (te) at (4, 9) {TE};
% 		\node [f2] (expse) at (6, 9) {Exp-SE};
	    
% 	    \node [f2] (nde) at (3, 7) {NDE};
% 		\node [f2] (nie) at (5, 7) {NIE};
		
% 		\node (gap) [draw,rectangle,minimum width=6cm,minimum height=3.5cm] at (5,8) {};
	    
% 		\node [f2] (sde) at (3, 5) {S-DE};
% 		\node [f2] (sie) at (5, 5) {S-IE};
% 		\node [f2] (sse) at (7, 5) {S-SE};
		
% 		\node [f1] (scm) at (5, 3) {SCM $\mathcal{M}$};

% 		% arrows/edges
% 		\draw (scm) to (sde);
% 		\draw (scm) to (sie);
% 		\draw (scm) to (sse);
		
% 		\draw (sde) to (nde);
% 		\draw (sie) to (nie);
% 		\draw (sse) to (expse);
		
% 		\draw (nde) to (te);
% 		\draw (nie) to (te);
		
% 		\draw (te) to (tv);
% 		\draw (expse) to (tv);

% 	\end{tikzpicture}
% \caption{Bridging the gap between total variation (TV) and the SCM.}
% \vspace{-0.4in}
% \label{fig:gapsolved}
% \end{wrapfigure}
\begin{definition}[Total and spurious effects] \label{def:teexpse}
    Let the total effect and experimental spurious effect be defined as follows:
\begin{align}
    \text{TE}_{x_0, x_1}(y) &= P(y_{x_1}) - P(y_{x_0}) \\
    \text{Exp-SE}_{x}(y) &= P(y_{x}) - P(y \mid x)
\end{align}
We write TE-fair$_X(Y)$ whenever $\text{TE}_{x_0, x_1}(y) = 0$, or simply TE-fair when $X$ and $Y$ are clear from the context. Exp-SE-fair is defined analogously.
\end{definition}
In words, TE measures the difference in the outcome $Y$ when setting $X = x_1$, compared to setting $X = x_0$ by intervention. The measure can be visualized graphically as shown in Fig.~\ref{fig:graphTE}. In the context of the COMPAS dataset in Ex.~\ref{ex:compas}, total effect would be the average difference in recidivism prediction when setting an individuals race to White compared to setting their race to Non-White. Experimental spurious effect measures the average difference in outcome $Y$ when setting $X = x$ by intervention, compared to simply observing that $X = x$, as shown graphically in Fig.~\ref{fig:graphExpSE}. In COMPAS, this would mean the average difference in recidivism prediction for individuals for whom the race is set to White by intervention, compared to simply observing the race to be White.  
Based on these two notions, the TV can be decomposed into two distinct sources of variation, which correspond precisely to causal and non-causal mechanisms:
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
             \begin{tikzpicture}
	 [>=stealth, rv/.style={thick}, rvc/.style={triangle, draw, thick, minimum size=7mm}, node distance=18mm]
	 \pgfsetarrows{latex-latex};
		\node[rv] (z1) at (0,1) {$Z$};
	 	%\node[rv] (x1) at (-1.5,0) {$X$};
	 	
	 	\node[rv] (x1x) at (-1,0) {$X=x_1$};
	 	
	 	\node[rv] (w1) at (0,-1) {$W$};
	 	\node[rv] (y1) at (1.5,0) {$Y$};
	 	
	 	\draw[->] (x1x) -- (w1);
		\draw[->] (z1) -- (y1);
	 	\path[->] (x1x) edge[bend left = 0] (y1);
		%\path[<->] (x1) edge[bend left = 30, dashed] (z1);
	 	\draw[->] (w1) -- (y1);
		\draw[->] (z1) -- (w1);
		
		\node (mns) at (2.25, 0) {\Large $-$};
		\node (a) at (0, -1.5) {$P(y_{x_1})$};
		\node (b) at (4.5, -1.5) {$P(y_{x_0})$};
		
		\node[rv] (z2) at (4.5,1) {$Z$};
	 	%\node[rv] (x2) at (3,0) {$X$};
	 	\node[rv] (x2x) at (3.5,0) {$X=x_0$};
	 	\node[rv] (w2) at (4.5,-1) {$W$};
	 	\node[rv] (y2) at (6,0) {$Y$};
	 	
	 	\draw[->] (x2x) -- (w2);
		\draw[->] (z2) -- (y2);
	 	\path[->] (x2x) edge[bend left = 0] (y2);
		%\path[<->] (x2) edge[bend left = 30, dashed] (z2);
	 	\draw[->] (w2) -- (y2);
		\draw[->] (z2) -- (w2);
	 \end{tikzpicture}
\caption{Total effect TE$_{x_0, x_1}(y)$.}
\label{fig:graphTE}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
             \begin{tikzpicture}
	 [>=stealth, rv/.style={thick}, rvc/.style={triangle, draw, thick, minimum size=7mm}, node distance=18mm]
	 \pgfsetarrows{latex-latex};
		\node[rv] (z1) at (0,1) {$Z$};
	 	%\node[rv] (x1) at (-1.5,0) {$X$};
	 	
	 	\node[rv] (x1x) at (-1,0) {$X=x$};
	 	
	 	\node[rv] (w1) at (0,-1) {$W$};
	 	\node[rv] (y1) at (1.5,0) {$Y$};
	 	
	 	\draw[->] (x1x) -- (w1);
		\draw[->] (z1) -- (y1);
	 	\path[->] (x1x) edge[bend left = 0] (y1);
		%\path[<->] (x1) edge[bend left = 30, dashed] (z1);
	 	\draw[->] (w1) -- (y1);
		\draw[->] (z1) -- (w1);
		
		\node (mns) at (2.25, 0) {\Large $-$};
		\node (a) at (0, -1.5) {$P(y_{x})$};
		\node (b) at (4.5, -1.5) {$P(y \mid x)$};
		
		\node[rv] (z2) at (4.5,1) {$Z$};
	 	\node[rv] (x2) at (3.5,0) {$X=x$};
	 	\node[rv] (w2) at (4.5,-1) {$W$};
	 	\node[rv] (y2) at (6,0) {$Y$};
	 	
	 	\draw[->] (x2) -- (w2);
		\draw[->] (z2) -- (y2);
	 	\path[->] (x2) edge[bend left = 0] (y2);
		\path[<->] (x2) edge[bend left = 30, dashed] (z2);
	 	\draw[->] (w2) -- (y2);
		\draw[->] (z2) -- (w2);
	 \end{tikzpicture}
\caption{Experimental spurious effect Exp-SE$_{x}(y)$.}
\label{fig:graphExpSE}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \begin{tikzpicture}
	 [>=stealth, rv/.style={thick}, rvc/.style={triangle, draw, thick, minimum size=7mm}, node distance=18mm]
	 \pgfsetarrows{latex-latex};
		\node[rv] (z1) at (0,1) {$Z$};
	 	%\node[rv] (x1) at (-1.5,0) {$X$};
	 	
	 	\node[rv] (x11) at (-1.1,0.3) {$X=x_1$};
	 	\node[rv] (x10) at (-1.1,-0.3) {$X=x_0$};
	 	
	 	\node[rv] (w1) at (0,-1) {$W$};
	 	\node[rv] (y1) at (1.5,0) {$Y$};
	 	
	 	\draw[->] (x10) -- (w1);
		\draw[->] (z1) -- (y1);
	 	\path[->] (x11) edge[bend left = 0] (y1);
		%\path[<->] (x1) edge[bend left = 30, dashed] (z1);
	 	\draw[->] (w1) -- (y1);
		\draw[->] (z1) -- (w1);
		
		\node (mns) at (2.25, 0) {\Large $-$};
		\node (a) at (0, -1.5) {$P(y_{x_1, W_{x_0}})$};
		\node (b) at (4.5, -1.5) {$P(y_{x_0})$};
		
		\node[rv] (z2) at (4.5,1) {$Z$};
	 	%\node[rv] (x2) at (3,0) {$X$};
	 	\node[rv] (x20) at (3.5,0) {$X=x_0$};
	 	\node[rv] (w2) at (4.5,-1) {$W$};
	 	\node[rv] (y2) at (6,0) {$Y$};
	 	
	 	\draw[->] (x20) -- (w2);
		\draw[->] (z2) -- (y2);
	 	\path[->] (x20) edge[bend left = 0] (y2);
		%\path[<->] (x2) edge[bend left = 30, dashed] (z2);
	 	\draw[->] (w2) -- (y2);
		\draw[->] (z2) -- (w2);
	 \end{tikzpicture}
         \caption{Natural direct effect NDE$_{x_0, x_1}(y)$.}
         \label{fig:graphNDE}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \begin{tikzpicture}
	 [>=stealth, rv/.style={thick}, rvc/.style={triangle, draw, thick, minimum size=7mm}, node distance=18mm]
	 \pgfsetarrows{latex-latex};
		\node[rv] (z1) at (0,1) {$Z$};
	 	%\node[rv] (x1) at (-1.5,0) {$X$};
	 	
	 	\node[rv] (x11) at (-1.1,0.3) {$X=x_1$};
	 	\node[rv] (x10) at (-1.1,-0.3) {$X=x_0$};
	 	
	 	\node[rv] (w1) at (0,-1) {$W$};
	 	\node[rv] (y1) at (1.5,0) {$Y$};
	 	
	 	\draw[->] (x10) -- (w1);
		\draw[->] (z1) -- (y1);
	 	\path[->] (x11) edge[bend left = 0] (y1);
		%\path[<->] (x1) edge[bend left = 30, dashed] (z1);
	 	\draw[->] (w1) -- (y1);
		\draw[->] (z1) -- (w1);
		
		\node (mns) at (2.25, 0) {\Large $-$};
		\node (a) at (0, -1.5) {$P(y_{x_1, W_{x_0}})$};
		\node (b) at (4.5, -1.5) {$P(y_{x_1})$};
		
		\node[rv] (z2) at (4.5,1) {$Z$};
	 	%\node[rv] (x2) at (3,0) {$X$};
	 	\node[rv] (x20) at (3.5,0) {$X=x_1$};
	 	\node[rv] (w2) at (4.5,-1) {$W$};
	 	\node[rv] (y2) at (6,0) {$Y$};
	 	
	 	\draw[->] (x20) -- (w2);
		\draw[->] (z2) -- (y2);
	 	\path[->] (x20) edge[bend left = 0] (y2);
		%\path[<->] (x2) edge[bend left = 30, dashed] (z2);
	 	\draw[->] (w2) -- (y2);
		\draw[->] (z2) -- (w2);
	 \end{tikzpicture}
        \caption{Natural indirect effect NIE$_{x_1, x_0}(y)$.}
        \label{fig:graphNIE}
     \end{subfigure}
     \caption{Graphical representations of measures used in TV$_{x_0, x_1}(y)$ decomposition.}
     \label{fig:graphMeasures}
\end{figure}
\begin{lemma}[TV decomposition I] \label{lemma:te+expse}
The total variation measure can be decomposed as
\begin{align}
    \text{TV}_{x_0, x_1}(y) =  \text{TE}_{x_0, x_1}(y) + (\text{Exp-SE}_{x_0}(y) - \text{Exp-SE}_{x_1}(y)).
\end{align}
\end{lemma}
Lem. \ref{lemma:te+expse} shows how the TV measure can be decomposed into causal and non-causal variations. In fact, the TV measure equals the total effect with a transition from $X = x_0$ to $X = x_1$ plus the experimental spurious effect of $X = x_0$ minus the experimental spurious effect of $X = x_1$.

Interestingly, note that the total effect captures any kind of causal influence of $X$ on $Y$, be it direct or indirect. Based on the doctrines of disparate treatment and impact, or otherwise, we might be interested in whether a causal effect is a direct consequence of the protected attribute, or is perhaps mediated by other variables. In other words, the TE measure is also composite and therefore will not be admissible with respect to direct and indirect structural fairness criteria, so we want to further decompose it. In the literature, total effect is often decomposed into measures known as the natural direct and indirect effects \citep{pearl2013direct}, which are defined as:
\begin{definition}[Natural direct and indirect effects \citep{pearl2013direct}] \label{def:ndenie}
    The natural direct and indirect are defined, respectively, as:
    \begin{align}
        \text{NDE}_{x_0, x_1}(y) = P(y_{x_1, W_{x_0}}) - P(y_{x_0}) \\
        \text{NIE}_{x_1, x_0}(y) = P(y_{x_1, W_{x_0}}) - P(y_{x_1}).
    \end{align}
We write NDE-fair$_X(Y)$ for NDE$_{x_0, x_1}(y) = 0$, or simply NDE-fair when the attribute and outcome are clear from the context. The condition NIE-fair is defined analogously.
\end{definition}
In words, the NDE captures the difference in outcome $Y$ when setting $X = x_1$, but keeping the mediators $W$ at the value they would attain naturally under $X = x_0$ intervention, compared to setting $X = x_0$ by intervention. In the context of our COMPAS example, the NDE would measure how much the predicted probability of recidivism would have changed for an individual whose race was set by intervention to White, had their race been set to Non-White, but their juvenile and prior offense counts took a value they would have attained naturally (that is, a value naturally attained when setting the race to White). This definition is illustrated in Fig.~\ref{fig:graphNDE}. 

The definition of NIE follows a similar logic. In this case, we consider a change in outcome $Y$ that occurs when setting $X=x_0$, while keeping $X=x_1$ to its naturally attained value along the direct causal pathway, as shown in Fig.~\ref{fig:graphNIE}. For the COMPAS example, the NIE would measure how much the predicted probability of recidivism would have changed for an individual whose race was set to White, had their race been set to Non-White along the indirect causal pathway influencing the values of juvenile and prior offense counts. By applying the decomposition into natural direct and indirect effects, we obtain the following corollary:
\begin{corollary}[TV decomposition II] \label{cor:expsendenie}
The total variation measure can be decomposed as
    \begin{align}
        \text{TV}_{x_0, x_1}(y) &= \text{NDE}_{x_0, x_1}(y) - \text{NIE}_{x_1, x_0}(y) + (\text{Exp-SE}_{x_0}(y) - \text{Exp-SE}_{x_1}(y)).
    \end{align}
\end{corollary}
In words, the TV measure can be written as the natural direct effect with a transition from $X = x_0$ to $X = x_1$ minus the natural indirect effect with the opposite transition plus the experimental spurious effect of $X = x_0$ minus the experimental spurious effect of $X = x_1$. Using the structural basis expansion from Thm.~\ref{thm:contrasts} these measures can be expanded as:
\begin{align} 
    \label{eq:tedown}
    \text{TE}_{x_0, x_1}(y) &= \sum_u [y_{x_1}(u) - y_{x_0}(u)]P(u) \\
    \label{eq:expseup}
    \text{Exp-SE}_{x}(y) &= \sum_u y_{x}(u)[P(u) - P(u\mid x)] \\
    \label{eq:ndedown}
    \text{NDE}_{x_0, x_1}(y) &= \sum_u [y_{x_1, W_{x_0}}(u) - y_{x_0}(u)]P(u) \\
    \label{eq:ctfiedown}
    \text{NIE}_{x_1, x_0}(y) &= \sum_u [y_{x_1, W_{x_0}}(u) - y_{x_1}(u)]P(u).
\end{align}
It is also important to see whether measures appearing in Cor.~\ref{cor:expsendenie} are admissible for capturing discrimination on a structural level (following Def.~\ref{def:str-fair}). To this end, we make the following claim:
\begin{corollary} \label{cor:admissible}
    The fairness criteria based on NDE, NIE, and Exp-SE measures are admissible with respect to structural direct, indirect and spurious fairness (S-DE, S-IE, S-SE) respectively. The total variation measure is not admissible with respect to any of the three structural fairness criteria. Additionally, the criteria based on NDE, NIE and Exp-SE put together are more powerful than the TV based criterion. Formally, these facts are written as:
    \begin{align}
        \text{S-DE} &\implies \text{NDE-fair} \label{eq:admnde}\\
        \text{S-IE} &\implies \text{NIE-fair} \label{eq:admnie}\\
        \text{S-SE} &\implies \text{Exp-SE-fair}\label{eq:admexpse}.
    \end{align}
Finally, putting the NDE, NIE and Exp-SE measures together implies the TV measure is equal to $0$:
\begin{equation}
    \text{NDE-fair} \wedge \text{NIE-fair} \wedge \text{Exp-SE-fair} \implies \text{TV-fair}.
\end{equation}
\end{corollary}
An important practical implication of the admissibility relations in Cor.\ref{cor:admissible} is the following. The contrapositive of Eq.~\ref{eq:admnde} implies that:
\begin{equation}
    (\text{NDE}_{x_0, x_1}(y) \neq 0) \implies  \neg \text{S-DE}. 
\end{equation}
Based on this, one can test the following hypothesis:
\begin{align}
    H_0: \text{NDE}_{x_0, x_1}(y) = 0.
\end{align}
If the $H_0$ hypothesis is rejected, a data scientist can conclude that direct discrimination is present in the dataset. In contrast, a hypothesis test based on the TV is not sufficient to test for existence of a direct effect. Additionally, Cor.~\ref{cor:admissible} shows that by decomposing TV we obtained measures that are, put together, strictly more informative than TV. Fig.~\ref{fig:babymap} shows how we can place the measures from Def.~\ref{def:teexpse} and \ref{def:ndenie} along the population and mechanism axes that were introduced in Sec.~\ref{foundations} (Fig.~\ref{fig:Erefined}). A natural question is whether the measures shown in Fig.~\ref{fig:babymap} are sufficient for Causal Fairness Analysis, or if other, more powerful measures are necessary. To see why more powerful measures of fairness are needed, we offer an example.
\tikzstyle{fairmap}=[
	every node/.style={draw=none, align=center, fill=none, text centered, anchor=center,font=\it},
	every label/.style={font=\small, text = red},
	cx/.append style={anchor=center,sloped,rotate=90,text=red,font=\bf,pos=0.65},
	f1/.style={draw=,fill=gray!15,thick,inner sep=3pt,minimum width=2.5em, align=center, text centered},
	imp/.style={double,->},
]
\renewcommand{\myx}{1.6}
\renewcommand{\myy}{-1.6}
\definecolor{colone}{RGB}{99,172,229}
\definecolor{coltwo}{RGB}{231, 239,246}
\definecolor{colthree}{RGB}{173,203,227}
\begin{figure}
	\centering
	\begin{tikzpicture}[fairmap]
		
		\draw [very thin] (\myx, 0.5 * \myy) -- (9 * \myx, 0.5 * \myy);
		\draw [very thin, -{Latex[length=3mm]}] (0, 0) -- node[above, rotate=90]{population axis} (0, 2.2 * \myy);
		\draw [very thin, -{Latex[length=3mm]}] (0, 0) -- node[above]{mechanism axis} (9.25*\myx, 0);
		
		\draw [very thin] (\myx, 1.5 * \myy) -- (9 * \myx, 1.5*\myy);
		
		\draw [very thin] (\myx,0) -- (\myx, 1.5*\myy);
		\draw [very thin] (3*\myx,0) -- (3*\myx, 1.5*\myy);
		\draw [very thin] (5*\myx,0) -- (5*\myx, 1.5*\myy);
		\draw [very thin] (7*\myx,0) -- (7*\myx, 1.5*\myy);
		\draw [very thin] (9*\myx,0) -- (9*\myx, 1.5*\myy);
		
		\node [draw=red, rotate=90] at (0.5*\myx, \myy)  {$P(u)$};
		
		\node [f1] (tv) at (0.5*\myx, 0.25*\myy) {TV};
        
        \node (spurious) at (4 * \myx, 0.25*\myy) {Spurious};
        \node [f1] (exp-se) at (4*\myx, \myy) {Exp-SE};
        \node [f1] (se) at (4*\myx, 2*\myy) {S-SE};
        
        \node (causal) at (2 * \myx, 0.25*\myy) {Causal};
        \node [f1] (te) at (2*\myx, \myy) {TE};
        \node [f1] (ce) at (2*\myx, 2*\myy) {S-TE};
        
        \node (direct) at (6 * \myx, 0.25*\myy) {Direct};
        \node [f1] (nde) at (6*\myx, \myy) {NDE};
        \node [f1] (de) at (6*\myx, 2*\myy) {S-DE};
        
        \node (indirect) at (8 * \myx, 0.25*\myy) {Indirect};
        \node [f1] (nie) at (8*\myx, \myy) {NIE};
        \node [f1] (ie) at (8*\myx, 2*\myy) {S-IE};

 		\node (te-se) at (1.25*\myx, 0.65*\myy) {$\wedge$};
 		\node (nde-nie) at (5.25 * \myx, 0.65*\myy) {$\wedge$};
        
        % join the ANDs
 		\draw [-] (te) to [bend left = 0] (te-se);
 		\draw [-] (exp-se) to [bend right = 10] (te-se);
 		
 		\draw [-] (nde) to [bend left = 20] (nde-nie);
 		\draw [-] (nie) to [bend right = 10] (nde-nie);
 		
 		% implications
 		\draw [imp] (te-se) to [bend right = 10] (tv);
 		\draw [imp] (nde-nie) to [bend right = 10] (te);
 		
 		\draw [imp] (se) to [bend left = 0] (exp-se);
		\draw [imp] (ie) to (nie);
		\draw [imp] (de) to (nde);
		\draw [imp] (ce) to (te);

	\end{tikzpicture}
	\caption{Placing the total, experimental spurious, natural direct, and natural indirect effects along the population and mechanism axes that were first introduced in Fig.~\ref{fig:Erefined}.}
	\label{fig:babymap}
\end{figure}

\begin{example}[Limitation of Natural Direct Effect] \label{ex:NDEfail}
Consider a startup company that is currently in hiring season. The hiring decision ($Y \in \lbrace 0,1\rbrace$ indicating whether the candidate is hired) is based on gender ($X \in \lbrace 0, 1\rbrace$ indicating female and male, respectively), age ($Z \in \lbrace 0, 1\rbrace$, indicating younger and older than 40 years, respectively), and education level ($W \in \lbrace 0, 1\rbrace$ indicating whether the applicant has a PhD). The true SCM $\mathcal{M}$, unknown to the data analyst, is given by:\\
\begin{align}
    \label{eq:ndefail1}
    U &\gets N(0, 1)\\
    X &\gets \text{Bernoulli}(expit(U))\\
    Z &\gets \text{Bernoulli}(expit(U)) \\
    W &\gets \text{Bernoulli}(0.3) \\
    \label{eq:ndefail2}
    Y &\gets \text{Bernoulli}(\frac{1}{5}(X + Z - 2XZ) + \frac{1}{6}W),
\end{align}
where expit$(x) = \frac{e^x}{1 + e^x}$. Using the fact that $Y_{x_1,W_{x_0}}$ is Bernoulli$(\frac{1}{5}(1-Z) + \frac{1}{6}W)$ and $Y_{x_0}$ is Bernoulli$(\frac{1}{5}Z + \frac{1}{6}W)$, we compute the natural direct effect and obtain that
\begin{align}
        \text{NDE}_{x_0, x_1}(y) &= P(y_{x_1, W_{x_0}}) - P(y_{x_0}) \\
                                &= P(\text{Bernoulli}(\frac{1}{5}(1-Z) + \frac{1}{6}W) = 1)\\ & - P(\text{Bernoulli}(\frac{1}{5}(Z) + \frac{1}{6}W) = 1)\nonumber\\
                                &= \sum_{z\in \lbrace 0,1\rbrace}\sum_{w \in \lbrace 0,1\rbrace} P(z, w)[\frac{1}{5}(1-z) + \frac{1}{6}w -\frac{1}{5}z - \frac{1}{6}w]\\
                                &= \sum_{z\in \lbrace 0,1\rbrace}\sum_{w \in \lbrace 0,1\rbrace} P(z)P(w) [\frac{1}{5}(1-2z)] \quad \text{since } P(z,w)=P(z)P(w) \\
                                &= \sum_{z\in \lbrace 0,1\rbrace} P(z)[\frac{1}{5}(1-2z)] = \frac{1}{2}\times\frac{1}{5} + \frac{1}{2}\times\frac{-1}{5} = 0. \label{eq:NDEfailmix}
\end{align}
However, note that structural direct effect is present, that is S-DE$_x(y)$ does not hold, since the outcome $Y$ is a function of gender $X$ in Eq.~\ref{eq:ndefail2}.
\end{example}
This example illustrates that even though the NDE is admissible with respect to structural direct effect, it can still happen that the NDE equals 0 and yet structural direct effect exists. The reader might have noticed that in this case the NDE is an aggregate measure over two distinct groups, as can be seen in Line~\ref{eq:NDEfailmix}. In fact, when considering junior applicants, females are 20\% less likely to be hired, whereas for senior applicants, males are 20\% less likely to be hired. This results in the cancellation of the two effects and the NDE equating to $0$, in turn making it impossible for the analyst to detect discrimination using only the NDE. The reason for this can also be seen when using the structural basis expansion of the NDE. In Eq.~\ref{eq:ndedown}, the posterior weighting term is $P(u)$, which means both younger and older applicants are included in the quantity. We next discuss measures suitable for determining discrimination within specific subgroups of the population (such as different age groups as above).
